Sidewalk Measurements from Satellite Images: Preliminary Findings

Large-scale analysis of pedestrian infrastructures, particularly sidewalks, is critical to human-centric urban planning and design. Benefiting from the rich data set of planimetric features and high-resolution orthoimages provided through the New York City Open Data portal, we train a computer vision model to detect sidewalks, roads, and buildings from remote-sensing imagery and achieve 83% mIoU over held-out test set. We apply shape analysis techniques to study different attributes of the extracted sidewalks. More specifically, we do a tile-wise analysis of the width, angle, and curvature of sidewalks, which aside from their general impacts on walkability and accessibility of urban areas, are known to have significant roles in the mobility of wheelchair users. The preliminary results are promising, glimpsing the potential of the proposed approach to be adopted in different cities, enabling researchers and practitioners to have a more vivid picture of the pedestrian realm.

==> review.tex <==
SUBMISSION: 13
TITLE: Sidewalk measurements from satellite images: Preliminary findings


----------------------- REVIEW 1 ---------------------
SUBMISSION: 13
TITLE: Sidewalk measurements from satellite images: Preliminary findings
AUTHORS: Maryam Hosseini, Iago B. Araujo, Hamed Yazdanpanah, Eric Tokuda, Fabio Miranda, Claudio T. Silva and Roberto M. Cesar Jr.

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
This paper proposed a framework for semantic segmentation of sidewalks. Sidewalks are always noticeably overlooked. 

This is a good research point on the sidewalks detection.
However, the authors had not stated the difficulties on sidewalk measurement compared to other roads. 
The framework is too simple, it is a process more than a framework. it's hard to found the new contributions.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 13
TITLE: Sidewalk measurements from satellite images: Preliminary findings
AUTHORS: Maryam Hosseini, Iago B. Araujo, Hamed Yazdanpanah, Eric Tokuda, Fabio Miranda, Claudio T. Silva and Roberto M. Cesar Jr.

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
In this submission the authors present a semantic segmentation approach to identifying sidewalks and their various components.  The researchers present a test case in New York City and report on the accuracy of their results.  Overall the paper is very well structured and well written.  I have outlined a few comments below that may help to improve the submission.

Planimetric data is typically manually digitized from aerial imagery (though this is changing) or manually collected through surveying.  Was this true for your dataset?  Is the planimetric data simply lines or polygon representations of the sidewalks?  Further details on the actual planimetric data itself would be useful.

The discussion about how angle and curvature of the sidewalk is determined is a bit dense and difficult to follow in places.  A figure might be useful here.

What was the source of the aerial images? <to be added> 

These are impressive results given the occlusion in many cases. 

Given that Manhattan contains prototypical American city rectangular blocks with straight streets, I would be curious to hear the authors’ thoughts on the generalizability of this model. 
What would happen if you were to pick this up and apply it to a city in Europe with far less regular blocks and few straight streets?

----------------------- REVIEW 3 ---------------------
SUBMISSION: 13
TITLE: Sidewalk measurements from satellite images: Preliminary findings
AUTHORS: Maryam Hosseini, Iago B. Araujo, Hamed Yazdanpanah, Eric Tokuda, Fabio Miranda, Claudio T. Silva and Roberto M. Cesar Jr.

----------- Overall evaluation -----------
SCORE: 3 (strong accept)
----- TEXT:
The paper is very interesting with potentially extensive impact. It seeks to introduce a framework to identify sidewalks from aerial images. The existing literature, research gaps and aim are clearly stated and discussed. The contributions are clearly identified. The results are clearly explained and discussed. Yet they are very brief - arguably because of word limit requirements. I look forward to learning more about this research.
